Pedestrian Attribute Recognition: A New Benchmark Dataset and A Large Language Model Augmented Framework

Pedestrian Attribute Recognition (PAR) is one of the indispensable tasks in human-centered research. However, existing datasets neglect different domains (e.g., environments, times, populations, and data sources), only conducting simple random splits, and the performance of these datasets has already approached saturation. In the past five years, no large-scale dataset has been opened to the public. To address this issue, this paper proposes a new large-scale, cross-domain pedestrian attribute recognition dataset to fill the data gap, termed MSP60K. It consists of 60,122 images and 57 attribute annotations across eight scenarios. Synthetic degradation is also conducted to further narrow the gap between the dataset and real-world challenging scenarios. To establish a more rigorous benchmark, we evaluate 17 representative PAR models under both random and cross-domain split protocols on our dataset. Additionally, we propose an innovative Large Language Model (LLM) augmented PAR framework, named LLM-PAR. This framework processes pedestrian images through a Vision Transformer (ViT) backbone to extract features and introduces a multi-embedding query Transformer to learn partial-aware features for attribute classification. Significantly, we enhance this framework with LLM for ensemble learning and visual feature augmentation. Comprehensive experiments across multiple PAR benchmark datasets have thoroughly validated the efficacy of our proposed framework. The dataset and source code accompanying this paper will be made publicly available at \url{https://github.com/Event-AHU/OpenPAR}.

==> ____.tex <==


% As detailed in Table~\ref{division}, the dataset is divided in two ways: the first is random partitioning with a training set of 30,298 images, a validation set of 6,002 images, and a test set of 23,822 images, ensuring random distribution of scenes in each set. The second method is cross-domain partitioning, dividing the dataset into eight scenarios with five used for training and three for testing, allowing for the evaluation of domain generalization and zero-shot performance of the PAR method.

% Our research conduct a statistical analysis of the MSP60K pedestrian attribute recognition dataset, which comprises 60,122 images of pedestrians captured from 17 different locations, featuring over 5,000 unique individuals. As shown in Table~\ref{Publicdatasets}, we compare our dataset with the existing PAR benchmark datasets. It is emphasized that our dataset comprises 8 distinct scenes and 57 attributes, which provides more comprehensive annotations than datasets such as PA100k (26 attributes), and WIDER (14 attributes). The MSP60K dataset includes a variety of environments such as markets, schools, kitchens, ski resorts, various outdoor, and construction sites, contrasting with the more limited scope of other datasets. As detailed, the dataset is divided in two ways. The first method is random partitioning, which includes a training set of 30,298 images, a validation set of 6,002 images, and a test set of 23,822 images, ensuring a random distribution of scenes across each set. The second method is cross-domain partitioning, dividing the dataset into eight scenarios. Five of these scenarios are used for training, specifically \textbf{ Construction Site}, \textbf{Market}, \textbf{Kitchens}, \textbf{School}, and \textbf{Ski Resort}, with a total of 34,128 images. The remaining three scenarios, \textbf{Outdoors1}, \textbf{Outdoors2}, and \textbf{Outdoors3}, with a total of 24,994 images, are used for testing. This partitioning method allows for the evaluation of domain generalization and zero-shot performance of the PAR method. To validate model robustness in complex environments, we degrade 1/3 of the data in each subset, including variations such as lighting changes, random occlusions, blurring, and noise. With 60,015 images, MSP60K offers a substantial dataset size, contributing to a better understanding and evaluation of PAR methods in diverse and realistic conditions.




% \begin{table}[!htb]
% \center
% \small  
% \caption{Details of Random Split and Cross-domain Split of our MSP60K dataset.} 
% \label{division} 
% \begin{tabular}{c|c|c|c}
% \hline \toprule [0.5 pt]
% \multicolumn{1}{c|}{\multirow{1}{*}{\textbf{Partition}}} &  \multicolumn{1}{c|}{\multirow{1}{*}{\textbf{Set}}} & \multicolumn{1}{c|}{\textbf{Domain}}  & \multicolumn{1}{c}{\textbf{\#Image}} \\
% \hline    
% \multirow{3}{*}{Random}  & Train & Random & 30298 \\ 
%                          & Val & Random & 6002 \\ 
%                          & Test & Random & 23822 \\ 
% \hline
% \multirow{8}{*}{Cross-domain}    & \multirow{5}{*}{Train}    & Constuction Site & 4403 \\ 
%                                 &                             & Market & 17384 \\ 
%                                 &                            & Kitchens & 1665\\ 
%                                 &                            & School & 5896 \\ 
%                                 &                            & Ski Resort & 5780 \\ \cline{2-4}                          
%                                 & \multirow{3}{*}{Test}     & Outdoors1 & 8788 \\ 
%                                 &                            & Outdoors2 & 4657 \\ 
%                                 &                            & Outdoors3 & 11549 \\     
% \hline \toprule [0.5 pt] 

% \end{tabular} 
% \end{table}

% \textbf{Attribute-Guide Adaptive Fusion.} 
% % 为了高效综合三个分支的优势，我们提出Attribute-Guide Adaptive Fusion策略，我们在训练集使用模型推理得到三个分支的预测概率集合$P = [ P_{ILC}, P_{ILC}, P_{TC}]$，我们对三个分支的预测进行分分数计算，
% To efficiently integrate the strengths of the three branches, we propose the Attribute-Guide Adaptive Fusion strategy. During training, we use the model to infer the predicted probability sets from the three branches, $P = [P_{ALC}, P_{ILC}, P_{TC}]$, and calculate scores for each branch predictions, we collect scores $S^M_{m=1} = [ scores_{ALC}, scores_{ILC}, scores_{TC}]$ from branch training results, where $M$ represents the number of metrics used to evaluate the branches. We define the the best branch as $ \bold I^M_{m=1} = \{ i_1,i_2,\dots,i_a\}$, obtained by using $\arg\max$ on $S^M_{m=1}$ with a representing the number of attributes. The fusion weights $W$ are calculated as follows:
% \begin{equation}\label{weight_calculation}
%     W = \mathbbm{1}(\forall_{m=1}^M \, \bold I_m = i) \cdot e^i + (1 - \mathbbm{1}(\forall_{m=1}^M \, \bold I_m = i) ) \cdot \omega(\bold I^M)
% \end{equation}
% where $e^i$  is a vector with 1 in the i-th position and 0 elsewhere, and $\omega(\bold I^M) = [ p_{ALC}, p_{ILC}, p_{TC}]$ , with the $p$ obtained by applying softmax to the improvement values of the highest-scoring branches when there are discrepancies in the metrics. The indicator function $\mathbbm{1}( \forall_{m=1}^M \, \bold I_m = i )$  equals 1 if all metrics indicate that a particular branch is the best and 0 otherwise. In our approach, we use Accuracy and F1-score as the evaluation metrics for determining the fusion weights.

% Our classifier consists of three components: an attribute-level visual classifier, an instance-level classifier, and a text classifier. Our method offers significant improvements, unlike previous pedestrian attribute recognition frameworks that rely solely on visual data or a simple visual-language fusion approach~\cite{fan2023parformer,2022drformer, wang2023pedestrian}. Purely visual methods struggle to use contextual information about attributes effectively. Although visual-language fusion methods model relationships between attributes, basic fusion modules often fail to capture the true meaning of attribute vocabulary, relying instead on inductive biases from the training data. In contrast, our approach uses a multimodal large language model to perform deeper semantic reasoning, combining images and descriptive text to provide a more comprehensive visual understanding.

% \textbf{Attributes-Level Classifier (Attr-CLS).} This classifier assigns a dedicated classifier to each attribute, using Convolutional Block Attention Modules (CBAM) to capture fine-grained features. The features are then mapped to attribute-specific predictions $P_{attr}$ through a fully connected layer.

% \textbf{Instance-Level Classifier (IN-CLS).} To address the dataset's long-tail distribution, this classifier assigns one classifier per attribute group, sharing features to improve generalization. It maps CBAM-aggregated features to attribute groups, allowing rare attributes to benefit from common ones. The combined predictions from multiple groups result in instance-level predictions $P_{in}$.

% \textbf{LLM Classifier (LLM-CLS).}
% The above two classifiers directly classify visual features, making it difficult to perform semantic inference by using contextual information about attributes. To address this, we use the hidden layer states from the LLM as the input for the text classifier. The LLM provides attribute classification based on contextual relationships, supplementing the lack of contextual linkage in pure visual classifiers. The LLM branch's predicted probabilities are $P_{llm}$.

% The previous classification frameworks based on MLLM, such as GMM~\cite{} use text and category similarity matching. However, it's challenging to determine a matching similarity threshold due to the uncertain number of pedestrian attributes in PAR task. To enhance recognition by effectively utilizing the contextual and semantic information of LLMs, we use the hidden states output by the LLM as the basis for classification. Specifically, we first divide the instruction $T$ by \textit{$<$ImageHere$>$}, and pass it through the tokenizer and embedding layers of the LLM, obtain multiple sets of instruction embeddings $T_E = { T_E^1, T_E^2, \dots, T_E^{k+1} }$. Next, we insert the corresponding visual features into these embeddings and concatenate them to form the initial instruction feature $F_I$. During training phase, we embed the ground truth and concatenate it to $F_I$ as the initial input of the LLM, using the right-shifted ground truth as the supervision label. After passing through the LLM, $F_I$ produces hidden states $F_H$, which are then processed by both a classification head and a language head to generate two outputs: the classification head output directly maps to the predefined attribute list $A$, yielding language classification logits $P_{llm}$; the language head output maps to the vocabulary and, after applying softmax, computes the language loss $L_{llm}$ against the ground truth labels.

% During our training process, we identified that prematurely introducing the ground truth accelerates training but compromises the learning of the LLM classification head due to information leakage. To address this, we implemented a ground truth substitution strategy that avoids complete ground truth introduction during training, ensuring optimal learning of the LLM classification head. We use a template to expand pedestrian attributes into sentences: \textit{The \{Age\} \{Gender\} \{Hair\}, \{Orientations\} wearing \{Upper Body\} on tops, and \{Lower Body\} on bottoms, and is carrying \{Bags\}. He is \{Action\}.} This template, along with the modified instructions, forms the $<$instruction, answer$>$ set.
%  We also utilize the ground truth mask strategy to prevent information leakage during training, which helps in effectively learning the LLM classification head. Additionally, we employ a template to expand pedestrian attributes into sentences for training, creating the $<$instruction, answer$>$ set.

% 我们的分类器包括属性级别视觉分类器、实例级别分类器和文本分类器。为有效融合多个分支的优势，我们提出了Attribute-Guide Adaptive Fusion（AGAFW），以属性级别的表现集成每个分支的结果。与以往的纯视觉和视觉-语言融合的行人属性识别框架不同，纯视觉方案难以有效利用属性的上下文信息，而视觉-语言融合方法虽然建模了属性之间的联系，但简单的融合模块可能仅通过训练集获得归纳偏差，无法真正理解属性词汇的含义。因此，我们使用多模态大语言模型进行深入的语义推理，结合图像和描述文本，提供更全面的视觉理解。

% To effectively integrate the strengths of these different branches, we propose the Attribute-Guide Adaptive Fusion (AGAF). AGAF integrates the results from each branch based on their performance at the attribute level, ensuring a comprehensive fusion of their capabilities.

% 如Tabel ~\ref{ablation}所示，我们对我们方法中的各个组件进行了分析，主要有视觉主干分析，AGFA模块，语言增强分支，实例增强分支。视觉主干分析是为了更加清晰的表明我们视觉分支对于我们方法表现的贡献，并且为了验证我们基于MLLMs的一系列微调改进是有效的，我们也提供了MiniGPT-4在多个数据集上的zero-shot性能分析，我们直接将MiniGPT-4生成的文本经过BERT后使用一个分类器得到分类结果。
% 当仅有EVA-CLIP和微调的Q-Former, mA、Acc和F1分别达到了82.89、72.32和81.89。为了更有效的挖掘视觉主干的潜力并且不破坏其泛化能力，我们引入Lora微调来适应我们的任务，加入LoRATune后，模型的mA、Acc和F1分别达到了90.14、83.25和89.38。为了证明LLM和纯视觉分类之间互补性，我们进一步引入LLM分支（不包含AGFA模块）时，mA、Acc和F1分别达到了90.89、83.64和89.60。加入AGFA模块后，mA、Acc和F1分别达到了92.20、83.76和89.70。这说明提出的AGFA属性组特征聚合模块在特征聚合方面的有效性，能够进一步提升模型的识别能力。并且使用MLLMs增强行人属性识别是有效的，视觉分支和LLM分支之间存在互补性。最后，我们评估了CLS-IN模块的效果。加入实例分支后，mA、Acc和F1分别提升了0.22，0.12和0.13，说明了实例分支通过共享特征的学习，提升了对尾部类别的识别能力，并补充了其他类别。



% \begin{table}[!htb]
% \center
% \setlength{\tabcolsep}{3pt}
% \small 
% \caption{Comparison with state-of-the-art methods on RAPv1 datasets. The \textcolor{red}{first} and \textcolor{blue}{second} are shown in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively. "-" means this indicator is not available.} \label{Comparisononrapdatasets} 
% \resizebox{0.45\textwidth}{!}{%
% \begin{tabular}{l|ccccc}
% \hline \toprule [0.5 pt]
% \multicolumn{1}{c|}{\multirow{2}{*}{Methods}} & \multicolumn{5}{c}{RAPv1} \\ \cline{2-6} 
% \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c}{mA} &
%   \multicolumn{1}{c}{Acc} &
%   \multicolumn{1}{c}{Prec} &
%   \multicolumn{1}{c}{Recall} &
%   \multicolumn{1}{c}{F1} \\ \hline
% SSCsoft\cite{2021ssc} & 82.77 & 68.37 & 75.05 & 87.49 & 80.43\\
% IAA-Caps\cite{2022iaacaps} & 81.72 & 68.47 & 79.56 & 82.06 & 80.37\\
% MCFL \cite{Chen2022MCFL} & 84.04 & 67.28 & 73.44 &87.75 & 79.96\\
% DRFormer \cite{2022drformer} & 81.81 &70.60 & 80.12 & 82.77 & 81.42\\
% VAC \cite{guo2022visual} & 81.30 & 70.12 &81.56 & 81.51 &81.54\\
% DAFL\cite{jia2022learning} & 83.72 & 68.18 & 77.41 & 83.39 & 80.29  \\
% CGCN \cite{Fan2022CGCN} &84.70 & 54.40 & 60.03 & 83.68 & 70.49 \\ 
% CAS\cite{yang2021cascaded} & 84.18 & 68.59 & 77.56 & 83.81 & 80.56\\ 
% VTB \cite{cheng2022VTB} & 82.67 & 69.44 & 78.28 & 84.39 & 80.84 \\
% PromptPAR \cite{wang2023pedestrian}  &85.45 &71.61 & 79.64 & 86.05 &82.38  \\
% PARFormer \cite{fan2023parformer}  &84.43 &69.94 & 79.63 & 88.19 &81.35 \\
% OAGCN~\cite{lu2023oagcn}   &87.83 &69.32 &78.32 &87.29 &82.56 \\
% SSPNet \cite{SHEN2024110194} & 83.24 & 70.21 & 80.14 & 82.90 & 81.50 \\
% SOFAFormer \cite{wu2024selective} &83.40 &70.00 &80.00 &83.00 &81.20   \\
% FRDL\cite{zhou2024pedestrian} &87.72 &- &- &- &79.16 \\
% \hline 
% Zero-shot & 65.46 & 50.90 & 64.48 & 65.20 & 66.06 \\
% Ours(ViT-B/16) &  &  &  &  &  \\ 
% Ours(ViT-L/14) &  &  &  &  &   \\ 
% Ours(ViT-G/14) & 86.67 &  &  &  & 83.16 \\
% \hline \toprule [0.5 pt] 
% \end{tabular}}
% \end{table}


% % 如Tabel ~\ref{ablation}所示，我们对我们方法中的各个组件进行了消融实验，如视觉主干分析，AGFA模块，语言增强分支，实例增强分支。视觉主干分析是为了更加清晰的表明我们视觉分支对于我们方法表现的贡献，并且为了验证我们基于MLLMs的一系列微调改进是有效的，我们也提供了MiniGPT-4在多个数据集上的zero-shot性能分析，我们直接将MiniGPT-4生成的文本经过BERT后使用一个分类器得到分类结果。
% As shown in Table~\ref{ablation}, we conducted ablation experiments on various components of our method, including visual backbone analysis, the AGFA module, the language enhancement branch, and the instance enhancement branch. The visual backbone analysis aims to clearly demonstrate the contribution of our visual branch to the performance of our method. Additionally, to verify the effectiveness of our series of fine-tuning improvements based on MLLMs, we also provide zero-shot performance analysis of MiniGPT-4 on multiple datasets. We obtained classification results by directly passing the text generated by MiniGPT-4 through BERT and then using a classifier.

% \textbf{Effects of the Visual Backbone} 
% % 分析纯视觉主干性能 表明性能来源并不全是主干
% % 为了验证我们框架的表现不是完全依赖于视觉分类，我们首先对视觉主干进行了一系列的分析，以和加入我们组件进行对比。我们的视觉主干指的是EVA-CLIP和Q-Former, 只有视觉主干和Linear Prob时，模型的mA、Acc和F1分别为71.54、58.24和71.96，当微调Q-Former时，性能有一些改善，mA、Acc和F1分别达到了82.89、72.32和81.89。为了更有效的挖掘视觉主干的潜力并且不破坏其泛化能力，我们引入Lora微调来适应我们的任务， 加入LoRATune后，模型的mA、Acc和F1分别达到了90.14、83.25和89.38。
% To demonstrate that our proposed framework's performance is not solely reliant on visual classification, we first analyze the visual backbone and compare it with other results with additional components. Our visual backbone consists of EVA-CLIP and Q-Former. When using only the visual backbone and the Linear probe, the model achieves scores of 71.54 for mA, 58.24 for Acc, and 71.96 for F1, respectively. This shows that the performance is limited without other components, even though the visual backbone captures some pedestrian features. To improve the visual backbone and extract more corresponding attribute features, we fine-tune the Q-Former, resulting in enhancements with mA, Acc, and F1 scores reaching 82.89, 72.32, and 81.89, respectively. To more effectively harness the potential of the visual backbone without compromising its generalization ability,  we implemented LoRA fine-tuning to adjust it to our specific task. By adding LoRATune, the model's mA, Acc, and F1 scores improved to 90.14, 83.25, and 89.38, respectively.

% \textbf{Effects of Large Language Model}
% % 分析LLMs可以带来性能提升
% % 为了证明LLM和纯视觉分类之间互补性，我们进一步引入LLM分支（不包含AGFA模块）时，mA、Acc和F1分别达到了90.89、83.64和89.60。并且结合LLM分支和AGFA模块后，性能进一步提升到92.20、83.76和89.70。这些结果表明，使用LLMs增强行人属性识别是有效的，视觉分支和LLM分支之间存在互补性。
% To demonstrate the complementarity between LLM and pure visual classification, we further introduced the LLM branch (excluding the AGFA module). The mA, Acc, and F1 scores reached 90.89, 83.64, and 89.60, respectively. When combining the LLM branch with the AGFA module, the performance further improved to 92.20, 83.76, and 89.70. These results indicate that enhancing pedestrian attribute recognition with LLMs is effective, and there is a complementary relationship between the visual branch and the LLM branch.


% \textbf{Effects of AGFA Module}
% % 分析提出的模块有效性
% % 在分析AGFA（Attributes Group Features Aggregation）模块的效果时，我们观察到其在引入LLM的基础上进一步提升了性能。加入AGFA模块后，mA、Acc和F1分别达到了92.20、83.76和89.70。这说明提出的AGFA属性组特征聚合模块在特征聚合方面的有效性，能够进一步提升模型的识别能力。
% When analyzing the effectiveness of the AGFA (Attributes Group Features Aggregation) module, w observed that it further improved performance when introduced on top of the LLM. With the addition of the AGFA module, the mA, Acc, and F1 scores reached 92.20, 83.76, and 89.70, respectively. This demonstrates the effectiveness of the proposed AGFA module in feature aggregation, significantly enhancing the model's recognition capabilities.
% % \textbf{Effects of CLS-V}
% % % 我们分析了仅使用语言分支的性能表现，可以看到仅使用语言分支

% \textbf{Effects of CLS-IN}
% % 最后，我们评估了CLS-IN模块的效果。加入实例分支后，mA、Acc和F1分别提升了0.22，0.12和0.13，说明了实例分支通过共享特征的学习，提升了对尾部类别的识别能力，并补充了其他类别。
% Finally, we evaluated the effectiveness of the CLS-IN module. After adding the instance branch, the mA, Acc, and F1 scores improved by 0.22, 0.12, and 0.13, respectively. This indicates that the instance branch enhances the recognition of tail categories through shared feature learning and supplements the recognition of other categories.


% $\bullet$ \noindent \textbf{Analysis on the Number of AGFA Layers.}
% % 在这个工作中我们提出了AGFA用于提取属性组特征的行人特征。如表~\ref{CrossLayers}, 我们分析了1,3,6,9,12层的AGFA模块对于识别性能的影响，可以发现随着AGFA模块层数增强，相应的识别性能也会提升。但是处于计算负担的考虑，我们选择了3层的AGFA模块，在性能下降不严重的情况下，最大化计算效率。

% Layer & Querys
% \begin{table}[!htb]
% \center
% \small
% \caption{Comparing Cross Layers.} \label{layers}
% \begin{tabular}{c|c|c|c|c|c}
% \hline \toprule [0.5 pt]
% \multicolumn{1}{c|}{Layers} & \multicolumn{1}{c|}{1} & \multicolumn{1}{c|}{3} & \multicolumn{1}{c|}{6} & \multicolumn{1}{c|}{9}  & \multicolumn{1}{c}{12}  \\ \hline

% mA             & 91.92 & 92.20 & 92.52 & 92.63 & 92.72\\ \hline
% F1             & 89.45 & 90.02 & 90.24 & 90.32 & 90.16  \\ 
% \hline \toprule [0.5 pt]
% \end{tabular}
% \end{table}

% \begin{table}[!htb]
% \center
% \small
% \caption{Comparing query number of AGFA} \label{querys}
% \begin{tabular}{l|c|c|c}
% \hline \toprule [0.5 pt]
% \multicolumn{1}{c|}{Numbers} & \multicolumn{1}{c|}{256} & \multicolumn{1}{c|}{128} & \multicolumn{1}{c}{64}  \\ \hline
% mA             & 92.20 & 92.67 & 92.01 \\ \hline
% F1             & 90.02 & 90.16 & 88.28  \\ 
% \hline \toprule [0.5 pt]
% \end{tabular}
% \end{table}


% \begin{table}[]
% \center
% \small
% \caption{Comparing LoRA Dimension.} \label{LoRA}
% \begin{tabular}{c|c|c|c|c|c}
% \hline \toprule [0.5 pt]
% \multicolumn{1}{c|}{LoRA Dimention} & \multicolumn{1}{c|}{8} & \multicolumn{1}{c|}{16} & \multicolumn{1}{c|}{32} & \multicolumn{1}{c|}{64} \\ \hline

% mA             &   &    &  92.42  &    &     \\ \hline
% F1             &   &    &  89.83  &    &     \\ 
% \hline \toprule [0.5 pt]
% \end{tabular}
% \end{table}




% \begin{table}[]
% \center
% \small
% \caption{Lora fine-tuning the last K layers of LLM} \label{Cross Layers}
% \begin{tabular}{c|c|c}
% \hline \toprule [0.5 pt]
% \multicolumn{1}{c|}{K} & \multicolumn{1}{c|}{mA} & \multicolumn{1}{c}{F1} \\ \hline
% 0  &   &  \\
% 1  &   &  \\
% 2  &   &  \\
% 3  &   &  \\
% 4  &   &  \\
% \hline \toprule [0.5 pt]
% \end{tabular}
% \end{table}

